Quantum Effects in Cosmology

Quantum effects play an essential role in modern cosmology. Perhaps the most striking example comes from large-scale structures, generally assumed to originate from vacuum quantum fluctuations and stretched by an expansion phase. Inflation is the leading paradigm in explaining this process. The various observational successes of inflationary models drive the scientific community into elaborating more and more stringent tests, which can simultaneously be used to probe beyond the simple slow-roll, single field inflation. However, inflation is not a theory, and going beyond inflation is a necessity. Various alternatives and/or complementary mechanisms to inflation have been invoked in the literature. The best-known cosmological models endowed with the capacity of explaining large-scale observations while avoiding the singularity form a class called non-singular bouncing models. The main features of these models are the presence of a contraction phase before expansion, and a never-vanishing scale factor. A non-singular bounce generally appears when quantum effects are part of the model, playing the role of a regulator leading to the avoidance of singularities. This thesis focuses on a Hamiltonian formulation of quantum effects in cosmology. We first explore stochastic perturbations in a collapsing universe. Then, we show that quantum cosmology with Bohmian mechanics resolves the initial singularity. Adding a non-minimal coupling of gravity with electromagnetism, we show that the generation of magnetic fields is possible. Finally, we apply the affine quantisation on the Brans-Dicke Theory, the prototype of modified gravity theories, and we discuss the quantum equivalence of the Jordan and Einstein frames within this framework. We show that in both frames a smooth bounce is expected, and that equivalence between frames holds at the quantum level.

==> sections/abstract.tex <==
Even though predictions from inflationary models fit observations with great accuracy, inflation is not a theory, and it is therefore important to look at alternative mechanisms whose phenomenology can be constrained by cosmological data. It is possible to explain the origin of large-scale structures through bouncing models, taking into account the evolution of quantum perturbations in both a contracting phase and an expansion phase.\\

This thesis is motivated by the effects of quantum perturbations on cosmological models. We first focus on a semi-classical description of quantum perturbations in the form of stochastic noise in a collapsing universe. The growth of perturbations is a fundamental issue in bouncing cosmologies that any acceptable model must treat accurately. To this end, we quantified how quantum perturbations may overcome the classical energy density in the simple case of a massless field with exponential potential. This is generally not the case within this configuration, although there is an important growth of quantum diffusion in the case of a matter-dominated model, which could possibly drive the system away from the classical evolution. This stochastic collapse is the first step towards a complete stochastic bouncing model.\\

Numerous non-singular bouncing models resolve the initial singularity issue thanks to quantum effects. They constitute a broad class of relevant cosmological models, since they solve many problems of standard inflation. A subclass is obtained by considering the canonical quantisation of general relativity using the de Broglie-Bohm interpretation of quantum mechanics. In the second part of the thesis, we show that the generation of magnetic fields in such models compatible with observations on cosmological scales can be obtained with a simple coupling between gravity and electromagnetism. Interestingly, bouncing magnetogenesis have intrinsically less issues than inflationary magnetogenesis. The model presented here shows that acceptable magnetic fields can be obtained, depending on the energy scale of the coupling and the time when the bounce occurs.\\

To close the thesis, we finish with a bouncing model obtained from the affine quantisation of the Brans-Dicke theory. Contrary to canonical quantisation, the affine procedure needs less assumptions and kinetic energy terms possess a quantum potential regularising the dynamics, resulting in a smooth bounce. Another advantage of this method lies in the choice of mathematical models one can use to tackle the same physical problem. We employ this asset to deal with the quantum equivalence of Jordan and Einstein frames, an issue of modified gravity models. The results point toward an unitary equivalence of the frames. We conclude with a summary of achievements.\\

\textbf{Keywords:} cosmology, inflation, bouncing models, alternative to inflation, stochastic collapse, primordial magnetogenesis, affine quantisation.




==> sections/acknowledgements.tex <==
\chapter*{Acknowledgments / Agradecimentos}

First, I would like to thank my supervisor Nelson Pinto-Neto. Nelson's passion for physics along with his great sense of humour have made my stay in Rio very productive but at the same time very refreshing! I have always felt free to pursue the research I was interested in, and this made me grow a sense of independence necessary to an academic career. He made me discover some of the best locations in Rio (Adega da Velha!), where I hope we will meet again soon!

\vspace{0.4cm}

I sincerely thank my second supervisor David Wands for the year I stayed in Portsmouth. David is very enthusiastic about sharing his scientific knowledge, and is always preoccupied with the well-being of his students. He always makes himself available to discuss, and patiently taught me the rigour necessary to the production of a scientific paper.  I have also learnt tons of things about British history, like the story in which the French army was defeated by Admiral Nelson, as well as very interesting hidden pubs such as The George Inn!


%\vspace{0.8cm}
%
%I am very thankful to ... for accepting of being a part of my thesis examining board. I am grateful for their keen interest in my work.

\vspace{0.8cm}

I am extremely grateful to my collaborators Roberto Beneduci, Jean-Pierre Gazeau, Santiago Perez-Bergliaffa, Amedeo Perri and Sandro Vitenti, from whom I have learnt and am still learning a lot. I would like to show a lot of gratitude especially to Carla Almeida, my friend and collaborator, who reached out for me with the idea of initiating a (still ongoing!) collaboration that I hope will last for a long time!

\vspace{0.8cm}

I want to thank in particular Júlio Fabris, coordinator of the PPGCosmo program in which I enrolled, and the Department of Physics from the Universidade Federal do Espírito Santo. I wish to thank the University of Portsmouth for offering me ideal conditions of work during my year at the Institute of Cosmology and Gravitation. I would also like to give a special thank to the Centro Brasileiro de Pesquisas Físicas, where a consequent amount of work was done.

\vspace{0.8cm}

I wish to say thank you to Edison, Jhonny and Leo, my fellow CosmoSala students when I first arrived in Brazil and Denis, Heinrich, Olesya, Oliver, Pedro, Rodrigo, for making my stay in Vitória a very pleasant memory. I also wish to thank Chico and Elizabeth, my office mates in Rio and Bruno, Felipe, Guilherme, Luiz Felipe, Martin and Nelson, with whom I enjoyed a lot of animated conversations! Also a big thank you to Andrius, Ben, Bill, Chen, Chris, David, Julian, Laura, Matt, Michael, Mike, Natalie, Rob, for making my stay in Portsmouth a delight!

\vspace{0.8cm}

Finally, I want to thank Tays for staying by my side wherever we went, and for her endless love and support, and my family, who never ceased to encourage me. I love you all very dearly.


==> sections/resumo.tex <==
Mesmo que as previsões dos modelos inflacionários se encaixem nas observações com grande precisão, a inflação não é uma teoria e, portanto, é importante olhar para mecanismos alternativos cuja fenomenologia pode ser restringida por dados cosmológicos. É possível explicar a origem das estruturas de grande escala por meio de modelos de ricochete, levando em consideração a evolução das perturbações quânticas tanto em uma fase de contração quanto em uma fase de expansão.\\

Esta tese é motivada pelos efeitos de perturbações quânticas em modelos cosmológicos. Primeiramente, focamos em uma descrição semiclássica de perturbações quânticas na forma de ruído estocástico em um universo em colapso. O crescimento de perturbações é uma questão fundamental em cosmologias de ricochete que qualquer modelo aceitável deve tratar com precisão. Para tanto, quantificamos como as perturbações quânticas podem superar a densidade de energia clássica no caso simples de um campo sem massa com potencial exponencial. Esse geralmente não é o caso dentro desta configuração, embora haja um importante crescimento da difusão quântica no caso de um modelo dominado pela matéria, o que poderia possivelmente afastar o sistema da evolução clássica. Este colapso estocástico é o primeiro passo para um modelo de ricochete estocástico completo.\\

Numerosos modelos de ricochete não singulares resolvem o problema da singularidade inicial graças aos efeitos quânticos. Eles constituem uma ampla classe de modelos cosmológicos relevantes, uma vez que resolvem muitos problemas de inflação padrão. Uma subclasse é obtida considerando a quantização canônica da relatividade geral usando a interpretação de Broglie-Bohm da mecânica quântica. Na segunda parte da tese, mostramos que a geração de campos magnéticos em tais modelos compatíveis com observações em escalas cosmológicas pode ser obtida com um simples acoplamento entre gravidade e eletromagnetismo. Pode-se notar que a magnetogênese de ricochete tem intrinsecamente menos problemas do que a magnetogênese inflacionária. O modelo apresentado aqui mostra que campos magnéticos aceitáveis podem ser obtidos, dependendo da escala de energia do acoplamento e do tempo em que ocorre o salto.\\

Para encerrar a tese, finalizamos com um modelo de ricochete obtido a partir da quantização afim da teoria de Brans-Dicke. Ao contrário da quantização canônica, o procedimento afim precisa de menos hipóteses e os termos de energia cinética possuem um potencial quântico regularizando a dinâmica, resultando em um ricochete suave. Outra vantagem desse método está na escolha de modelos matemáticos que podem ser usados para discutir o mesmo problema físico. Consideramos essa vantagem para lidar com a equivalência quântica dos referenciais de Jordan e Einstein, uma questão de modelos de gravitação modificada. Os resultados apontam para uma equivalência unitária dos referenciais. Concluímos com um resumo dos resultados.\\

\textbf{Palavras-chave:} cosmologia, inflação, modelos de ricochete, alternativa à inflação, colapso estocástico, magnetogênese primordial, quantização afim.
